Autocalibration of a Mobile UWB Localization System for Ad-Hoc Multi-Robot Deployments in GNSS-Denied Environments

Ultra-wideband (UWB) wireless technology has seen an increased penetration in the robotics field as a robust localization method in recent years. UWB enables high accuracy distance estimation from time-of-flight measurements of wireless signals, even in non-line-of-sight measurements. UWB-based localization systems have been utilized in various types of GNSS-denied environments for ground or aerial autonomous robots. However, most of the existing solutions rely on a fixed and well-calibrated set of UWB nodes, or anchors, to estimate accurately the position of other mobile nodes, or tags, through multilateration. This limits the applicability of such systems for dynamic and ad-hoc deployments, such as post-disaster scenarios where the UWB anchors could be mounted on mobile robots to aid the navigation of UAVs or other robots. We introduce a collaborative algorithm for online autocalibration of anchor positions, enabling not only ad-hoc deployments but also movable anchors, based on Decawave's DWM1001 UWB module. Compared to the built-in autocalibration process from Decawave, we drastically reduce the amount of calibration time and increase the accuracy at the same time. We provide both experimental measurements and simulation results to demonstrate the usability of this algorithm.

==> anchor_pos3_errors_20200413_17_58_00.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color2}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{axis}[
axis background/.style={fill=white!82.7450980392157!black},
axis line style={white},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={Simulation Steps},
xmajorgrids,
xmin=-2.7, xmax=56.7,
xtick style={color=black},
y grid style={white},
ylabel={Anchor Position Error},
ymajorgrids,
ymin=-0.035177793909387, ymax=0.794510164560941,
ytick style={color=black},
ytick={-0.1,0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8},
yticklabels={-0.1,0.0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8}
]
\addplot [semithick, color0, mark=triangle*, mark size=2.5, mark options={solid}]
table {%
0 0.206851046053415
1 0.154347876211017
2 0.138284014767492
3 0.113123663655378
4 0.0760144271867652
5 0.075662327481571
6 0.141688775379064
7 0.182556291571946
8 0.206125664822357
9 0.275595159170825
10 0.113660970340444
11 0.141235286449457
12 0.195011759825975
13 0.252279801560074
14 0.351801879406218
15 0.41620817501599
16 0.500223042120859
17 0.548803769180824
18 0.627823943337199
19 0.648014464090219
20 0.138372388806015
21 0.0517523426850758
22 0.0159560569854024
23 0.00744898228315357
24 0.0723461495568029
25 0.139800787295395
26 0.188597190064554
27 0.238781982682829
28 0.278608011874944
29 0.305041451584314
30 0.208306409841597
31 0.242796280791257
32 0.282528748531445
33 0.35528860950468
34 0.433971544243946
35 0.478900980099165
36 0.544928251178398
37 0.558881861313129
38 0.596705622196207
39 0.675565744255077
40 0.394782175216273
41 0.447757656435988
42 0.462782236071579
43 0.484156952254601
44 0.530158947480038
45 0.555764647966367
46 0.595478755032179
47 0.643191473679806
48 0.69144155125668
49 0.748097856140475
50 0.507547878861749
51 0.547302637767373
52 0.622263750696723
53 0.715590144400659
54 0.733224101333921
};
\addlegendentry{A1}
\addplot [semithick, color1, mark=square*, mark size=2.5, mark options={solid}]
table {%
0 0.0509069778778193
1 0.098271147802479
2 0.145660265457198
3 0.204441350053135
4 0.216454444382665
5 0.308202629680602
6 0.386866873937604
7 0.459834037019173
8 0.550882677426749
9 0.604901196115664
10 0.0271080991563146
11 0.0302442030871435
12 0.114609120401124
13 0.153328406245146
14 0.219488990965708
15 0.289239207894307
16 0.371773497214999
17 0.425240564863432
18 0.433337747653285
19 0.475711718096086
20 0.0975361169368866
21 0.135209728655906
22 0.213989507222138
23 0.273137096379781
24 0.316687921509998
25 0.366575082862308
26 0.406444420918692
27 0.456590087090784
28 0.480558449074374
29 0.516604665629261
30 0.226122896102159
31 0.230360590251063
32 0.243098328144232
33 0.304499175665793
34 0.369404035177165
35 0.440238464479767
36 0.491256214816991
37 0.572156123328736
38 0.608522300302378
39 0.678169066179897
40 0.29008379818301
41 0.323679595370256
42 0.378772327433608
43 0.402456199381846
44 0.432318344463195
45 0.498462818347156
46 0.553751915696583
47 0.611006327815583
48 0.659832339409925
49 0.705139756583175
50 0.633411403307854
51 0.634345860007
52 0.637601219618554
53 0.683654810842249
54 0.706766029348294
};
\addlegendentry{A2}
\addplot [semithick, color2, mark=pentagon*, mark size=2.5, mark options={solid}]
table {%
0 0.23209712489548
1 0.198659141038607
2 0.109397420058705
3 0.0675201337455393
4 0.00253529511199157
5 0.0865627721514939
6 0.16492687980779
7 0.257375714339371
8 0.28414725121383
9 0.359661978653768
10 0.243137443271113
11 0.184867640764921
12 0.154459615105374
13 0.205367272637886
14 0.202526700267848
15 0.249719306896675
16 0.275336791270801
17 0.314324020120029
18 0.381201042248557
19 0.436124150814098
20 0.17679930867802
21 0.236576039887098
22 0.299933627090918
23 0.404124253501523
24 0.467709037020239
25 0.547975636932145
26 0.583149982437528
27 0.627963058422439
28 0.709355112377255
29 0.756797075539563
30 0.357165102964099
31 0.320440940168456
32 0.322027239653284
33 0.344238940848021
34 0.383034975336112
35 0.401443584558931
36 0.439266528162909
37 0.488332025701979
38 0.548431813511927
39 0.581314135157835
40 0.0806218654181425
41 0.040772992421317
42 0.064393261119794
43 0.140038052037301
44 0.212629093570606
45 0.251352377157624
46 0.303088545002927
47 0.355050808663066
48 0.388098236025024
49 0.433421429652515
50 0.484771204866125
51 0.412955920269276
52 0.360380015009365
53 0.297944657694334
54 0.306555172527727
};
\addlegendentry{A3}
\end{axis}

\end{tikzpicture}


==> boxplot_anchor_tag3_pos_error_20200413_17_58_09.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.752941176470588,0.796078431372549}
\definecolor{color1}{rgb}{0.67843137254902,0.847058823529412,0.901960784313726}

\begin{axis}[
axis line style={white},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={Positional Error},
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=2.5,
xtick style={color=black},
xtick={1,2},
xticklabels={Anchors,Tag},
y grid style={white!90!black},
ylabel={Error (m)},
ymajorgrids,
ymin=-0.035177793909387, ymax=0.794510164560941,
ytick style={color=black},
ytick={-0.1,0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8},
yticklabels={-0.1,0.0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8}
]
\addplot [black, forget plot]
table {%
1 0.205367272637886
1 0.00253529511199157
};
\addplot [black, forget plot]
table {%
1 0.498462818347156
1 0.756797075539563
};
\addplot [black, forget plot]
table {%
0.875 0.00253529511199157
1.125 0.00253529511199157
};
\addplot [black, forget plot]
table {%
0.875 0.756797075539563
1.125 0.756797075539563
};
\addplot [black, forget plot]
table {%
2 0.0585064405804479
2 0.00467971903596599
};
\addplot [black, forget plot]
table {%
2 0.143160109942574
2 0.222088616774788
};
\addplot [black, forget plot]
table {%
1.875 0.00467971903596599
2.125 0.00467971903596599
};
\addplot [black, forget plot]
table {%
1.875 0.222088616774788
2.125 0.222088616774788
};
\addplot [blue, mark=+, mark size=3, mark options={solid}, only marks, forget plot]
table {%
2 0.235457269384461
2 0.504050127928718
2 0.420858492042159
2 0.440032431475994
2 0.379530838537636
2 0.240411425256776
2 0.342096043133409
2 0.25124120071974
2 0.26145792733683
};
\path [draw=black, fill=color0]
(axis cs:0.75,0.205367272637886)
--(axis cs:1.25,0.205367272637886)
--(axis cs:1.25,0.498462818347156)
--(axis cs:0.75,0.498462818347156)
--(axis cs:0.75,0.205367272637886)
--cycle;
\path [draw=black, fill=color1]
(axis cs:1.75,0.0585064405804479)
--(axis cs:2.25,0.0585064405804479)
--(axis cs:2.25,0.143160109942574)
--(axis cs:1.75,0.143160109942574)
--(axis cs:1.75,0.0585064405804479)
--cycle;
\addplot [thick, black, forget plot]
table {%
0.75 0.351801879406218
1.25 0.351801879406218
};
\addplot [thick, black, forget plot]
table {%
1.75 0.0928596662046327
2.25 0.0928596662046327
};
\end{axis}

\end{tikzpicture}


==> boxplot_anchor_tag_pos_error_20200413_13_33_39.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.752941176470588,0.796078431372549}
\definecolor{color1}{rgb}{0.67843137254902,0.847058823529412,0.901960784313726}

\begin{axis}[
axis line style={white},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={Positional Error},
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=2.5,
xtick style={color=black},
xtick={1,2},
xticklabels={Anchors,Tag},
y grid style={white!90!black},
ylabel={Error (m)},
ymajorgrids,
ymin=-0.0354955273820243, ymax=0.873857146258537,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1},
yticklabels={-0.2,0.0,0.2,0.4,0.6,0.8,1.0}
]
\addplot [black, forget plot]
table {%
1 0.208987288578512
1 0.0498883200938622
};
\addplot [black, forget plot]
table {%
1 0.504281646043103
1 0.794553575131871
};
\addplot [black, forget plot]
table {%
0.875 0.0498883200938622
1.125 0.0498883200938622
};
\addplot [black, forget plot]
table {%
0.875 0.794553575131871
1.125 0.794553575131871
};
\addplot [blue, mark=+, mark size=3, mark options={solid}, only marks, forget plot]
table {%
1 0.83252293382033
1 0.820581298919768
};
\addplot [black, forget plot]
table {%
2 0.041416913006227
2 0.00583868505618303
};
\addplot [black, forget plot]
table {%
2 0.119000346166435
2 0.195152352804506
};
\addplot [black, forget plot]
table {%
1.875 0.00583868505618303
2.125 0.00583868505618303
};
\addplot [black, forget plot]
table {%
1.875 0.195152352804506
2.125 0.195152352804506
};
\addplot [blue, mark=+, mark size=3, mark options={solid}, only marks, forget plot]
table {%
2 0.418393129620582
2 0.206139760438463
2 0.358925529070999
2 0.220962332295537
2 0.256032289674816
2 0.369964540276474
};
\path [draw=black, fill=color0]
(axis cs:0.75,0.208987288578512)
--(axis cs:1.25,0.208987288578512)
--(axis cs:1.25,0.504281646043103)
--(axis cs:0.75,0.504281646043103)
--(axis cs:0.75,0.208987288578512)
--cycle;
\path [draw=black, fill=color1]
(axis cs:1.75,0.041416913006227)
--(axis cs:2.25,0.041416913006227)
--(axis cs:2.25,0.119000346166435)
--(axis cs:1.75,0.119000346166435)
--(axis cs:1.75,0.041416913006227)
--cycle;
\addplot [thick, black, forget plot]
table {%
0.75 0.32935461414297
1.25 0.32935461414297
};
\addplot [thick, black, forget plot]
table {%
1.75 0.0824992705586253
2.25 0.0824992705586253
};
\end{axis}

\end{tikzpicture}


==> concept/positioning.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color1}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color2}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color3}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color4}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
    name=ax1,
    height=\figureheight,
    width=\figurewidth,
    axis line style={white},
    legend cell align={left},
    legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
    tick align=outside,
    tick pos=left,
    x grid style={white},
    xmin=-3, xmax=38,
    xtick style={color=black},
    y grid style={white},
    ymin=-5, ymax=25,
    ytick style={color=black},
    axis line style={draw=none},
    tick style={draw=none},
    % put x-axis labels etc. on top
    % axis x line=top,
    % remove arrow tip
    % axis line style={-},
    % axis y line=none,
    % xmin=0,xmax=42,
    % ymin=0,ymax=42,
    % xlabel=stuff,
    xtick={5,10,15},
    ytick={5,10,15},
    xticklabels={,,},
    yticklabels={,,}
]
\draw[draw=color0] (axis cs:2,3) circle (10.7915821758131);
\path [draw=black, fill=color1, dashed]
(axis cs:9.00296327073541,11.0033865951262)
--(axis cs:9.00112886504206,10.9990122430882)
--(axis cs:9.00037628834735,10.9996707476961)
--(axis cs:2.00037628834735,2.99967074769607)
--(axis cs:1.99962371165265,3.00032925230393)
--(axis cs:8.99962371165265,11.0003292523039)
--(axis cs:8.99887113495794,11.0009877569118)
--cycle;
% \path [draw=black, fill=color1, dashed]
% (axis cs:9.00296327073541,11.0033865951262)
% --(axis cs:9.00112886504206,10.9990122430882)
% --(axis cs:9.00037628834735,10.9996707476961)
% --(axis cs:2.00037628834735,2.99967074769607)
% --(axis cs:1.99962371165265,3.00032925230393)
% --(axis cs:8.99962371165265,11.0003292523039)
% --(axis cs:8.99887113495794,11.0009877569118)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:11.0045,3)
% --(axis cs:11,2.9985)
% --(axis cs:11,2.9995)
% --(axis cs:2,2.9995)
% --(axis cs:2,3.0005)
% --(axis cs:11,3.0005)
% --(axis cs:11,3.0015)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:11.0045,3)
% --(axis cs:11,2.9985)
% --(axis cs:11,2.9995)
% --(axis cs:2,2.9995)
% --(axis cs:2,3.0005)
% --(axis cs:11,3.0005)
% --(axis cs:11,3.0015)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:18.0044229248412,6.00082929840773)
% --(axis cs:18.0002764328026,5.9985256917196)
% --(axis cs:18.0000921442675,5.99950856390653)
% --(axis cs:2.00009214426752,2.99950856390653)
% --(axis cs:1.99990785573247,3.00049143609347)
% --(axis cs:17.9999078557325,6.00049143609347)
% --(axis cs:17.9997235671974,6.0014743082804)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:18.0044229248412,6.00082929840773)
% --(axis cs:18.0002764328026,5.9985256917196)
% --(axis cs:18.0000921442675,5.99950856390653)
% --(axis cs:2.00009214426752,2.99950856390653)
% --(axis cs:1.99990785573247,3.00049143609347)
% --(axis cs:17.9999078557325,6.00049143609347)
% --(axis cs:17.9997235671974,6.0014743082804)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:15.0027335254841,20.0035746102484)
% --(axis cs:15.0011915367495,19.9990888248386)
% --(axis cs:15.0003971789165,19.9996962749462)
% --(axis cs:2.00039717891649,2.99969627494621)
% --(axis cs:1.99960282108351,3.00030372505379)
% --(axis cs:14.9996028210835,20.0003037250538)
% --(axis cs:14.9988084632505,20.0009111751614)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:15.0027335254841,20.0035746102484)
% --(axis cs:15.0011915367495,19.9990888248386)
% --(axis cs:15.0003971789165,19.9996962749462)
% --(axis cs:2.00039717891649,2.99969627494621)
% --(axis cs:1.99960282108351,3.00030372505379)
% --(axis cs:14.9996028210835,20.0003037250538)
% --(axis cs:14.9988084632505,20.0009111751614)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!62.7450980392157!black, dotted]
% (axis cs:4.00047108153033,22.0044752745381)
% --(axis cs:4.00149175817938,21.9998429728232)
% --(axis cs:4.00049725272646,21.9999476576077)
% --(axis cs:2.00049725272646,2.99994765760774)
% --(axis cs:1.99950274727354,3.00005234239226)
% --(axis cs:3.99950274727354,22.0000523423923)
% --(axis cs:3.99850824182062,22.0001570271768)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!62.7450980392157!black, dotted]
% (axis cs:4.00047108153033,22.0044752745381)
% --(axis cs:4.00149175817938,21.9998429728232)
% --(axis cs:4.00049725272646,21.9999476576077)
% --(axis cs:2.00049725272646,2.99994765760774)
% --(axis cs:1.99950274727354,3.00005234239226)
% --(axis cs:3.99950274727354,22.0000523423923)
% --(axis cs:3.99850824182062,22.0001570271768)
% --cycle;
\draw[draw=color1] (axis cs:11,3) circle (8.33252118184899);
\path [draw=black, fill=color1, dashed]
(axis cs:8.99890858968734,11.0043656412507)
--(axis cs:9.00145521375022,11.0003638034376)
--(axis cs:9.00048507125007,11.0001212678125)
--(axis cs:11.0004850712501,3.00012126781252)
--(axis cs:10.9995149287499,2.99987873218748)
--(axis cs:8.99951492874993,10.9998787321875)
--(axis cs:8.99854478624978,10.9996361965624)
--cycle;
% \path [draw=black, fill=color1, dashed]
% (axis cs:8.99890858968734,11.0043656412507)
% --(axis cs:9.00145521375022,11.0003638034376)
% --(axis cs:9.00048507125007,11.0001212678125)
% --(axis cs:11.0004850712501,3.00012126781252)
% --(axis cs:10.9995149287499,2.99987873218748)
% --(axis cs:8.99951492874993,10.9998787321875)
% --(axis cs:8.99854478624978,10.9996361965624)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:18.0041361526351,6.00177263684361)
% --(axis cs:18.0005908789479,5.99862128245497)
% --(axis cs:18.0001969596493,5.99954042748499)
% --(axis cs:11.0001969596493,2.99954042748499)
% --(axis cs:10.9998030403507,3.00045957251501)
% --(axis cs:17.9998030403507,6.00045957251501)
% --(axis cs:17.9994091210521,6.00137871754503)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:18.0041361526351,6.00177263684361)
% --(axis cs:18.0005908789479,5.99862128245497)
% --(axis cs:18.0001969596493,5.99954042748499)
% --(axis cs:11.0001969596493,2.99954042748499)
% --(axis cs:10.9998030403507,3.00045957251501)
% --(axis cs:17.9998030403507,6.00045957251501)
% --(axis cs:17.9994091210521,6.00137871754503)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:15.0010306770018,20.0043803772575)
% --(axis cs:15.0014601257525,19.9996564409994)
% --(axis cs:15.0004867085842,19.9998854803331)
% --(axis cs:11.0004867085842,2.99988548033314)
% --(axis cs:10.9995132914158,3.00011451966686)
% --(axis cs:14.9995132914158,20.0001145196669)
% --(axis cs:14.9985398742475,20.0003435590006)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:15.0010306770018,20.0043803772575)
% --(axis cs:15.0014601257525,19.9996564409994)
% --(axis cs:15.0004867085842,19.9998854803331)
% --(axis cs:11.0004867085842,2.99988548033314)
% --(axis cs:10.9995132914158,3.00011451966686)
% --(axis cs:14.9995132914158,20.0001145196669)
% --(axis cs:14.9985398742475,20.0003435590006)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:3.99844432588528,22.0042225440257)
% --(axis cs:4.00140751467523,22.0005185580382)
% --(axis cs:4.00046917155841,22.0001728526794)
% --(axis cs:11.0004691715584,3.00017285267941)
% --(axis cs:10.9995308284416,2.99982714732059)
% --(axis cs:3.99953082844159,21.9998271473206)
% --(axis cs:3.99859248532477,21.9994814419618)
% --cycle;
% \path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
% (axis cs:3.99844432588528,22.0042225440257)
% --(axis cs:4.00140751467523,22.0005185580382)
% --(axis cs:4.00046917155841,22.0001728526794)
% --(axis cs:11.0004691715584,3.00017285267941)
% --(axis cs:10.9995308284416,2.99982714732059)
% --(axis cs:3.99953082844159,21.9998271473206)
% --(axis cs:3.99859248532477,21.9994814419618)
% --cycle;
\draw[draw=color2] (axis cs:18,6) circle (10.3407899002729);
% \path [draw=black, fill=color1, dashed]
% (axis cs:8.99606629225745,11.0021853931903)
% --(axis cs:9.00072846439677,11.0013112359142)
% --(axis cs:9.00024282146559,11.0004370786381)
% --(axis cs:18.0002428214656,6.00043707863806)
% --(axis cs:17.9997571785344,5.99956292136194)
% --(axis cs:8.99975717853441,10.9995629213619)
% --(axis cs:8.99927153560323,10.9986887640858)
% --cycle;
% \path [draw=black, fill=color1, dashed]
% (axis cs:8.99606629225745,11.0021853931903)
% --(axis cs:9.00072846439677,11.0013112359142)
% --(axis cs:9.00024282146559,11.0004370786381)
% --(axis cs:18.0002428214656,6.00043707863806)
% --(axis cs:17.9997571785344,5.99956292136194)
% --(axis cs:8.99975717853441,10.9995629213619)
% --(axis cs:8.99927153560323,10.9986887640858)
% --cycle;
\path [draw=white!82.7450980392157!black, fill=white!82.7450980392157!black, dotted]
(axis cs:14.9990571191007,20.0044001108633)
--(axis cs:15.0014667036211,20.0003142936331)
--(axis cs:15.000488901207,20.0001047645444)
--(axis cs:18.000488901207,6.00010476454437)
--(axis cs:17.999511098793,5.99989523545563)
--(axis cs:14.999511098793,19.9998952354556)
--(axis cs:14.9985332963789,19.9996857063669)
--cycle;
% \path [draw=black, fill=color1, dotted]
% (axis cs:14.9990571191007,20.0044001108633)
% --(axis cs:15.0014667036211,20.0003142936331)
% --(axis cs:15.000488901207,20.0001047645444)
% --(axis cs:18.000488901207,6.00010476454437)
% --(axis cs:17.999511098793,5.99989523545563)
% --(axis cs:14.999511098793,19.9998952354556)
% --(axis cs:14.9985332963789,19.9996857063669)
% --cycle;
% \path [draw=black, fill=color1, dotted]
% (axis cs:3.99703672926459,22.0033865951262)
% --(axis cs:4.00112886504206,22.0009877569118)
% --(axis cs:4.00037628834735,22.0003292523039)
% --(axis cs:18.0003762883474,6.00032925230393)
% --(axis cs:17.9996237116526,5.99967074769607)
% --(axis cs:3.99962371165265,21.9996707476961)
% --(axis cs:3.99887113495794,21.9990122430882)
% --cycle;
% \path [draw=black, fill=color1, dotted]
% (axis cs:3.99703672926459,22.0033865951262)
% --(axis cs:4.00112886504206,22.0009877569118)
% --(axis cs:4.00037628834735,22.0003292523039)
% --(axis cs:18.0003762883474,6.00032925230393)
% --(axis cs:17.9996237116526,5.99967074769607)
% --(axis cs:3.99962371165265,21.9996707476961)
% --(axis cs:3.99887113495794,21.9990122430882)
% --cycle;
\draw[draw=color3] (axis cs:15,20) circle (10.8688955971015);
\path [draw=black, fill=color1, dashed]
(axis cs:8.99750384911699,10.9962557736755)
--(axis cs:8.99875192455849,11.0008320502943)
--(axis cs:8.99958397485283,11.0002773500981)
--(axis cs:14.9995839748528,20.0002773500981)
--(axis cs:15.0004160251472,19.9997226499019)
--(axis cs:9.00041602514717,10.9997226499019)
--(axis cs:9.00124807544151,10.9991679497057)
--cycle;
% \path [draw=black, fill=color1, dashed]
% (axis cs:8.99750384911699,10.9962557736755)
% --(axis cs:8.99875192455849,11.0008320502943)
% --(axis cs:8.99958397485283,11.0002773500981)
% --(axis cs:14.9995839748528,20.0002773500981)
% --(axis cs:15.0004160251472,19.9997226499019)
% --(axis cs:9.00041602514717,10.9997226499019)
% --(axis cs:9.00124807544151,10.9991679497057)
% --cycle;
\path [draw=black, fill=color1, dotted]
(axis cs:3.99557258540455,22.0008049844719)
--(axis cs:4.0002683281573,22.0014758048652)
--(axis cs:4.0000894427191,22.0004919349551)
--(axis cs:15.0000894427191,20.0004919349551)
--(axis cs:14.9999105572809,19.9995080650449)
--(axis cs:3.9999105572809,21.9995080650449)
--(axis cs:3.9997316718427,21.9985241951348)
% --cycle;
% \path [draw=black, fill=color1, dotted]
% (axis cs:3.99557258540455,22.0008049844719)
% --(axis cs:4.0002683281573,22.0014758048652)
% --(axis cs:4.0000894427191,22.0004919349551)
% --(axis cs:15.0000894427191,20.0004919349551)
% --(axis cs:14.9999105572809,19.9995080650449)
% --(axis cs:3.9999105572809,21.9995080650449)
% --(axis cs:3.9997316718427,21.9985241951348)
% --cycle;
\draw[draw=color4] (axis cs:4,22) circle (12.2409643218585);
\path [draw=black, fill=color1, dashed]
(axis cs:9.00186211324936,10.9959033508514)
--(axis cs:8.99863445028381,10.9993792955835)
--(axis cs:8.99954481676127,10.9997930985278)
--(axis cs:3.99954481676127,21.9997930985278)
--(axis cs:4.00045518323873,22.0002069014722)
--(axis cs:9.00045518323873,11.0002069014722)
--(axis cs:9.00136554971619,11.0006207044165)
--cycle;
% \path [draw=black, fill=color1, dashed]
% (axis cs:9.00186211324936,10.9959033508514)
% --(axis cs:8.99863445028381,10.9993792955835)
% --(axis cs:8.99954481676127,10.9997930985278)
% --(axis cs:3.99954481676127,21.9997930985278)
% --(axis cs:4.00045518323873,22.0002069014722)
% --(axis cs:9.00045518323873,11.0002069014722)
% --(axis cs:9.00136554971619,11.0006207044165)
% --cycle;
% \path [draw=black, fill=color1, dashed]
% (axis cs:9.00186211324936,10.9959033508514)
% --(axis cs:8.99863445028381,10.9993792955835)
% --(axis cs:8.99954481676127,10.9997930985278)
% --(axis cs:3.99954481676127,21.9997930985278)
% --(axis cs:4.00045518323873,22.0002069014722)
% --(axis cs:9.00045518323873,11.0002069014722)
% --(axis cs:9.00136554971619,11.0006207044165)
% --cycle;

% \path [draw=black, fill=color1, dashed]
% (axis cs:9.00186211324936,10.9959033508514)
% --(axis cs:8.99863445028381,10.9993792955835)
% --(axis cs:8.99954481676127,10.9997930985278)
% --(axis cs:3.99954481676127,21.9997930985278)
% --(axis cs:4.00045518323873,22.0002069014722)
% --(axis cs:9.00045518323873,11.0002069014722)
% --(axis cs:9.00136554971619,11.0006207044165)
% --cycle;

\addplot [semithick, color0, mark=square*, mark size=3, mark options={solid}, only marks]
table {%
2 3
};
\addlegendentry{Anchor 0}
\addplot [semithick, color1, mark=square*, mark size=3, mark options={solid}, only marks]
table {%
11 3
};
\addlegendentry{Anchor 1}
\addplot [semithick, color2, mark=square*, mark size=3, mark options={solid}, only marks]
table {%
18 6
};
\addlegendentry{Anchor 2}
\addplot [semithick, color3, mark=square*, mark size=3, mark options={solid}, only marks]
table {%
15 20
};
\addlegendentry{Anchor 3}
\addplot [semithick, color4, mark=square*, mark size=3, mark options={solid}, only marks]
table {%
4 22
};
\addlegendentry{Anchor 4}
\addplot [semithick, black, mark=triangle*, mark size=6, mark options={solid}, only marks]
table {%
9 11
};
\addlegendentry{Tag}
\addplot [semithick, white!82.7450980392157!black, dotted]
table {%
0 0
0.001 0.001
};
\addlegendentry{Autocalib.}
\addplot [semithick, black, dashed]
table {%
0 0
0.001 0.001
};
\addlegendentry{Tag Local.}
\end{axis}

\end{tikzpicture}


==> dists/real_meas_zoom.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis background/.style={fill=white!82.7450980392157!black},
    axis line style={white},
    legend cell align={left},
    legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
    tick align=outside,
    tick pos=left,
    x grid style={white},
    xlabel={Real Distance (m)},
    xmajorgrids,
    xmin=0.425, xmax=2.075,
    xtick style={color=black},
    xtick={0.4,0.6,0.8,1,1.2,1.4,1.6,1.8,2,2.2},
    xticklabels={0.4,0.6,0.8,1.0,1.2,1.4,1.6,1.8,2.0,2.2},
    y grid style={white},
    ylabel={Measured Distance (m)},
    ymajorgrids,
    ymin=0.700081707092281, ymax=2.45828415106211,
    ytick style={color=black},
    ytick={0.6,0.8,1,1.2,1.4,1.6,1.8,2,2.2,2.4,2.6},
    yticklabels={0.6,0.8,1.0,1.2,1.4,1.6,1.8,2.0,2.2,2.4,2.6}
]
\addplot [semithick, black]
table {%
0.5 0.865413404587226
0.6 0.966276901491704
0.7 1.06714039839618
0.8 1.16800389530066
0.9 1.26886739220514
1 1.36973088910961
1.2 1.57145788291857
1.4 1.77318487672752
1.6 1.97491187053648
1.8 2.17663886434543
2 2.37836585815439
};
\addlegendentry{Linear fit}
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
0.5 0.78
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
0.6 0.86
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
0.7 1.09
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
0.8 1.06
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
0.9 1.2
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
1 1.35
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
1.2 1.58
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
1.4 1.82
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
1.6 1.91
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}, forget plot]
table {%
1.8 2.1
};
\addplot [semithick, color0, mark=square*, mark size=1.42, mark options={solid}]
table {%
2 2.34
};
\addlegendentry{Raw data}
\end{axis}

\end{tikzpicture}


==> sections/05_Discussion.tex <==
\section{Discussion}

We have presented a mobile UWB-localization system with built-in autocalibration that can be deployed within a multi-robot system. The UWB anchors can be placed on mobile ground vehicles to support, for instance, the operation of UAVs and other robots in GNSS-denied environments. They key advantage of the proposed system is the periodic built-in self autocalibration of anchor positions. This allows for the localization error to stay within a certain tolerance even if the anchors are moving.

In future work, we will experiment with real multi-robot systems and provide a more exhaustive analysis on the usability of the proposed system in complex scenarios. We will also extend the calibration and localization approaches modelling the robots' dynamics and their odometry algorithms.


==> tags3_pos_error_20200413_17_58_01.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.854901960784314,0.647058823529412,0.125490196078431}
\definecolor{color1}{rgb}{0.980392156862745,0.501960784313725,0.447058823529412}
\definecolor{color2}{rgb}{0.627450980392157,0.32156862745098,0.176470588235294}

\begin{axis}[
axis background/.style={fill=white!82.7450980392157!black},
axis line style={white},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={Simulation Steps},
xmajorgrids,
xmin=-2.7, xmax=56.7,
xtick style={color=black},
y grid style={white},
ylabel={Tag Position Error},
ymajorgrids,
ymin=-0.0202888014086716, ymax=0.529018648373355,
ytick style={color=black},
ytick={-0.1,0,0.1,0.2,0.3,0.4,0.5,0.6},
yticklabels={-0.1,0.0,0.1,0.2,0.3,0.4,0.5,0.6}
]
\addplot [semithick, color0, mark=triangle*, mark size=4, mark options={solid,rotate=180}]
table {%
0 0.0462115096781704
1 0.121151376088916
2 0.14533613685534
3 0.0264101259677278
4 0.0472016350172657
5 0.0503879088301662
6 0.132636917449663
7 0.037783850181492
8 0.0264990123964002
9 0.0453668349682174
10 0.0222145503462213
11 0.0829791588585546
12 0.0753156590255472
13 0.0647648025475415
14 0.0453556634448395
15 0.0779552795052976
16 0.167458524192551
17 0.0331382278085554
18 0.133076238653665
19 0.0378133716914383
20 0.118478079083778
21 0.0642955655259322
22 0.440032431475994
23 0.161839133185005
24 0.0607483429477055
25 0.0420077559182508
26 0.0648243095430854
27 0.103285506754809
28 0.0507458816121294
29 0.0563920641931538
30 0.110144524800709
31 0.0576381234202858
32 0.176653641167803
33 0.0720444236335763
34 0.0788271178196612
35 0.155262085992848
36 0.0753849298311679
37 0.25124120071974
38 0.0894741003764399
39 0.124437502141063
40 0.102346432843062
41 0.112200137437861
42 0.1575252795674
43 0.0593391141223262
44 0.0590617774998406
45 0.26145792733683
46 0.0913906136850799
47 0.177889195953452
48 0.0388478755635993
49 0.173715151359671
50 0.121766119804244
51 0.172074255613131
52 0.188038951621647
53 0.124381574835447
54 0.137854627146669
};
\addlegendentry{Tag1}
\addplot [semithick, color1, mark=triangle*, mark size=4, mark options={solid}]
table {%
0 0.0100395695566515
1 0.00467971903596599
2 0.143032762946597
3 0.0133218907002928
4 0.0680066107898169
5 0.067403242730191
6 0.117417024194394
7 0.0665533569825459
8 0.0386058133681987
9 0.172104251795265
10 0.0585064405804479
11 0.19805749205475
12 0.0937066714799923
13 0.175124637467927
14 0.163214059421963
15 0.0941246888718799
16 0.0637231174748848
17 0.504050127928718
18 0.191126010166547
19 0.189575608242747
20 0.126075606469089
21 0.420858492042159
22 0.161947578368043
23 0.0770236866310498
24 0.0450036106864531
25 0.185065816525116
26 0.379530838537636
27 0.0340603086557159
28 0.0470278192451708
29 0.0661282260914493
30 0.240411425256776
31 0.168928436540779
32 0.168454244665881
33 0.0863720358341412
34 0.342096043133409
35 0.0274823730669747
36 0.131667221538174
37 0.0996217861719107
38 0.139306147543217
39 0.0525067646335392
40 0.0949998873472797
41 0.189148934044983
42 0.0975255163939895
43 0.207230800511162
44 0.210248948603282
45 0.114124790216024
46 0.05882058449724
47 0.0817760086790981
48 0.121310493747882
49 0.111435395338241
50 0.0801594213829878
51 0.120929902107156
52 0.0740784422531915
53 0.168662705499867
54 0.0997389170622713
};
\addlegendentry{Tag2}
\addplot [semithick, color2, mark=triangle*, mark size=4, mark options={solid,rotate=270}]
table {%
0 0.0769016933739431
1 0.0680663336857355
2 0.0534808121017522
3 0.0696926292688557
4 0.0286206249002351
5 0.118392095423411
6 0.0499520758494853
7 0.123266273705088
8 0.082020750202181
9 0.112661719757007
10 0.142129649402215
11 0.235457269384461
12 0.0914776880954947
13 0.0419784075266414
14 0.204730787950196
15 0.0942389884685361
16 0.0418750071618475
17 0.10719021241248
18 0.148488778897868
19 0.0464132559319273
20 0.0747922216776113
21 0.0693156049268132
22 0.191254201836127
23 0.128970613400911
24 0.0352866403012468
25 0.126471222833221
26 0.0928596662046327
27 0.053557396923184
28 0.0270336468341062
29 0.159232192165689
30 0.145346042038137
31 0.0553682511297993
32 0.0769090789051119
33 0.0441194267294822
34 0.0817111657861872
35 0.118827210960403
36 0.222088616774788
37 0.110002316012981
38 0.0833881441369552
39 0.1718652287899
40 0.143160109942574
41 0.062468444251477
42 0.190313045624931
43 0.0430228297504483
44 0.14192610623163
45 0.0795721667233979
46 0.0418421900272642
47 0.087889579610766
48 0.118760517942767
49 0.0319131032451077
50 0.0624004944975963
51 0.0488597785162212
52 0.128290095619435
53 0.0890911493282461
54 0.0448741616324064
};
\addlegendentry{Tag3}
\end{axis}

\end{tikzpicture}

